Abstracts or full text? Evaluating input scope and computational efficiency in biomedical lay summarization

Biomedical research articles are mainly written for experts and often contain terms that are difficult for the general public to understand. Automated lay summarization has become a solution to make biomedical knowledge easier for patients and the public to understand. However, generating lay summaries from full-text articles requires more computing power because the articles are long and costly to process. Fine-tuning large language models for this task also requires substantial resources. This study asks two questions: (1) whether abstracts contain enough information to produce lay summaries as good as those based on full-text articles, and (2) whether few-shot learning performs as well as task-specific fine-tuning. The study used two public biomedical lay summarization datasets and two recent models, evaluated for readability, factual consistency, semantic similarity, and runtime efficiency. Results show that abstract-based summarization performs better overall. Across both datasets and models, abstract fine-tuning is 4.70 times faster, while abstract zero- and few-shot prompting is 5.31 times faster than full-text methods. These results show that abstract-based prompting reduces runtime cost while maintaining lay summary quality.

==> macros.tex <==
\usepackage{graphicx}%
\usepackage{multirow}%
\usepackage{amsmath,amssymb,amsfonts}%
\usepackage{adjustbox}%
\usepackage{amsthm}%
\usepackage{mathrsfs}%
\usepackage{float}%
\usepackage[title]{appendix}%
\usepackage{textcomp}%
\usepackage{manyfoot}%
\usepackage{pgfplots}%
\usepackage{etoolbox}%
\usepackage{pgfplotstable}%
\usepackage{booktabs}%
\usepackage{algorithm}%
\usepackage{algorithmicx}%
\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{hyperref}%
%\usepackage[table,xcdraw]{xcolor}%
\usepackage{comment}%
\pgfplotsset{compat=1.18}%
\usepgfplotslibrary{statistics}%
\usepackage{pifont}
\usepackage[most]{tcolorbox}
\providecommand{\JournalTitle}[1]{#1}

\newcommand{\MinMax}[3]{%
  ( (#3) - (#2) < 1e-12 ? 0.5 : ( (#1) - (#2) ) / ((#3) - (#2)) )%
}
\newcommand{\MinMaxFlip}[3]{%
  1 - \MinMax{#1}{#2}{#3}%
}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\BoldIfEqFmt}[1]{%
  \pgfkeysgetvalue{/pgfplots/table/@cell content}\celltxt%
  \edef\celltxt{\celltxt}%
  \edef\maxtxt{#1}%
  \ifx\celltxt\maxtxt
    \pgfkeysalso{/pgfplots/table/@cell content/.add={\boldmath }{}}%
  \fi
}
\newcommand{\SmartTable}[3]{%
  \begingroup
  \pgfplotstableread[col sep=semicolon, row sep=\\]{%
Str;ROUGE;BLEU;METEOR;BERTScore;FKGL;DCRS;SMOG;CLI;SummaC;FENICE;FACTSCORE\\
MIN;#2\\
MAX;#3\\
#1
  }\datatable
  \pgfplotstablegetelem{0}{ROUGE}\of{\datatable}\let\ROUGEmin\pgfplotsretval
  \pgfplotstablegetelem{1}{ROUGE}\of{\datatable}\let\ROUGEmax\pgfplotsretval
  \pgfplotstablegetelem{0}{BLEU}\of{\datatable}\let\BLEUmin\pgfplotsretval
  \pgfplotstablegetelem{1}{BLEU}\of{\datatable}\let\BLEUmax\pgfplotsretval
  \pgfplotstablegetelem{0}{METEOR}\of{\datatable}\let\METEORmin\pgfplotsretval
  \pgfplotstablegetelem{1}{METEOR}\of{\datatable}\let\METEORmax\pgfplotsretval
  \pgfplotstablegetelem{0}{BERTScore}\of{\datatable}\let\BERTmin\pgfplotsretval
  \pgfplotstablegetelem{1}{BERTScore}\of{\datatable}\let\BERTmax\pgfplotsretval
  \pgfplotstablegetelem{0}{FKGL}\of{\datatable}\let\FKGLmin\pgfplotsretval
  \pgfplotstablegetelem{1}{FKGL}\of{\datatable}\let\FKGLmax\pgfplotsretval
  \pgfplotstablegetelem{0}{DCRS}\of{\datatable}\let\DCRSmin\pgfplotsretval
  \pgfplotstablegetelem{1}{DCRS}\of{\datatable}\let\DCRSmax\pgfplotsretval
  \pgfplotstablegetelem{0}{SMOG}\of{\datatable}\let\SMOGmin\pgfplotsretval
  \pgfplotstablegetelem{1}{SMOG}\of{\datatable}\let\SMOGmax\pgfplotsretval
  \pgfplotstablegetelem{0}{CLI}\of{\datatable}\let\CLImin\pgfplotsretval
  \pgfplotstablegetelem{1}{CLI}\of{\datatable}\let\CLImax\pgfplotsretval
  \pgfplotstablegetelem{0}{SummaC}\of{\datatable}\let\SUMMACmin\pgfplotsretval
  \pgfplotstablegetelem{1}{SummaC}\of{\datatable}\let\SUMMACmax\pgfplotsretval
  \pgfplotstablegetelem{0}{FENICE}\of{\datatable}\let\FENICEmin\pgfplotsretval
  \pgfplotstablegetelem{1}{FENICE}\of{\datatable}\let\FENICEmax\pgfplotsretval
  \pgfplotstablegetelem{0}{FACTSCORE}\of{\datatable}\let\FACTmin\pgfplotsretval
  \pgfplotstablegetelem{1}{FACTSCORE}\of{\datatable}\let\FACTmax\pgfplotsretval
  \pgfmathprintnumberto[fixed,precision=4]{\ROUGEmax}{\ROUGEmaxfmt}
  \pgfmathprintnumberto[fixed,precision=4]{\BLEUmax}{\BLEUmaxfmt}
  \pgfmathprintnumberto[fixed,precision=4]{\METEORmax}{\METEORmaxfmt}
  \pgfmathprintnumberto[fixed,precision=4]{\BERTmax}{\BERTmaxfmt}
  \pgfmathprintnumberto[fixed,precision=4]{\SUMMACmax}{\SUMMACmaxfmt}
  \pgfmathprintnumberto[fixed,precision=4]{\FENICEmax}{\FENICEmaxfmt}
  \pgfmathprintnumberto[fixed,precision=2]{\FKGLmin}{\FKGLminfmt}
  \pgfmathprintnumberto[fixed,precision=2]{\DCRSmin}{\DCRSminfmt}
  \pgfmathprintnumberto[fixed,precision=2]{\SMOGmin}{\SMOGminfmt}
  \pgfmathprintnumberto[fixed,precision=2]{\CLImin}{\CLIminfmt}
  \pgfmathsetmacro{\LongDocFactmax}{max(0, min(1, (\FACTmax + 10) / 10))}
  \pgfmathprintnumberto[fixed,precision=4]{\LongDocFactmax}{\LongDocFactmaxfmt}
  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{ROUGE}}{\ROUGEmin}{\ROUGEmax}}]{ROUGE_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{BLEU}}{\BLEUmin}{\BLEUmax}}]{BLEU_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{METEOR}}{\METEORmin}{\METEORmax}}]{METEOR_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{BERTScore}}{\BERTmin}{\BERTmax}}]{BERT_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMaxFlip{\thisrow{FKGL}}{\FKGLmin}{\FKGLmax}}]{FKGL_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMaxFlip{\thisrow{DCRS}}{\DCRSmin}{\DCRSmax}}]{DCRS_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMaxFlip{\thisrow{SMOG}}{\SMOGmin}{\SMOGmax}}]{SMOG_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMaxFlip{\thisrow{CLI}}{\CLImin}{\CLImax}}]{CLI_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{SummaC}}{\SUMMACmin}{\SUMMACmax}}]{SUMMAC_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{FENICE}}{\FENICEmin}{\FENICEmax}}]{FENICE_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{FACTSCORE}}{\FACTmin}{\FACTmax}}]{FACT_N}{\datatable}
  \pgfplotstablecreatecol[
    create col/expr={
      (\thisrow{ROUGE_N}+\thisrow{BLEU_N}+\thisrow{METEOR_N}+\thisrow{BERT_N}+
       \thisrow{FKGL_N}+\thisrow{DCRS_N}+\thisrow{SMOG_N}+\thisrow{CLI_N}+\thisrow{SUMMAC_N}+
       \thisrow{FENICE_N}+\thisrow{FACT_N})/11
    }
  ]{Mean}{\datatable}
  \pgfplotstablecreatecol[
    create col/expr={max(0, min(1, (\thisrow{FACTSCORE} + 10) / 10))}
  ]{LongDocFact}{\datatable}
  \pgfplotstablesort[
    sort key=Mean,
    sort cmp=float >,
    skip rows between index={0}{1}
  ]{\sorted}{\datatable}
  \pgfplotstabletypeset[
    row predicate/.code={%
      \pgfplotstablegetelem{\pgfplotstablerow}{Str}\of{\sorted}%
      \edef\cell{\pgfplotsretval}%
      \def\MINROW{MIN}%
      \def\MAXROW{MAX}%
      \ifx\cell\MINROW\pgfplotstableuserowfalse\fi
      \ifx\cell\MAXROW\pgfplotstableuserowfalse\fi
    },
    columns={Str,ROUGE,BLEU,METEOR,BERTScore,FKGL,DCRS,SMOG,CLI,SummaC,FENICE,LongDocFact,Mean},
    columns/Str/.style={string type, column name=Str},
    columns/ROUGE/.style={
      column name=ROUGE$\uparrow$, fixed, precision=4,
      postproc cell content/.append code={\BoldIfEqFmt{\ROUGEmaxfmt}}
    },
    columns/BLEU/.style={column name=BLEU$\uparrow$, fixed, precision=4,
      postproc cell content/.append code={\BoldIfEqFmt{\BLEUmaxfmt}}
    },
    columns/METEOR/.style={column name=METEOR$\uparrow$, fixed, precision=4,
      postproc cell content/.append code={\BoldIfEqFmt{\METEORmaxfmt}}
    },
    columns/BERTScore/.style={column name=BERTScore$\uparrow$, fixed, precision=4,
      postproc cell content/.append code={\BoldIfEqFmt{\BERTmaxfmt}}
    },
    columns/FKGL/.style={
      column name=FKGL$\downarrow$, fixed, precision=2,
      postproc cell content/.append code={\BoldIfEqFmt{\FKGLminfmt}}
    },
    columns/DCRS/.style={
      column name=DCRS$\downarrow$, fixed, precision=2,
      postproc cell content/.append code={\BoldIfEqFmt{\DCRSminfmt}}
    },
    columns/SMOG/.style={
      column name=SMOG$\downarrow$, fixed, precision=2,
      postproc cell content/.append code={\BoldIfEqFmt{\SMOGminfmt}}
    },
    columns/CLI/.style={
      column name=CLI$\downarrow$, fixed, precision=2,
      postproc cell content/.append code={\BoldIfEqFmt{\CLIminfmt}}
    },
    columns/SummaC/.style={column name=SummaC$\uparrow$, fixed, precision=4,
      postproc cell content/.append code={\BoldIfEqFmt{\SUMMACmaxfmt}}
    },
    columns/FENICE/.style={column name=FENICE$\uparrow$, fixed, precision=4,
      postproc cell content/.append code={\BoldIfEqFmt{\FENICEmaxfmt}}
    },
    columns/LongDocFact/.style={
      column name=LongDocFact$\uparrow$, fixed, precision=4,
      postproc cell content/.append code={\BoldIfEqFmt{\LongDocFactmaxfmt}}
    },
    columns/FACTSCORE/.style={fixed, precision=4},
    columns/Mean/.style={column name=Mean$\uparrow$, fixed, precision=4},
    every head row/.style={
      before row={
        \toprule
        & \multicolumn{4}{c}{Relevance}
        & \multicolumn{4}{c}{Readability}
        & \multicolumn{3}{c}{Factuality}
        & \\[-0.8ex]
        \cmidrule(lr){2-5}
        \cmidrule(lr){6-9}
        \cmidrule(lr){10-12}
      },
      after row=\midrule
    },
    every last row/.style={after row=\bottomrule},
    %font=\small
    font=\normalsize
  ]{\sorted}
  \endgroup
}

\newcommand{\SSITable}[1]{%
  \begingroup
  \pgfplotstableread[col sep=semicolon, row sep=\\]{#1}\datatable

  \pgfmathsetmacro{\SILmin}{999999} \pgfmathsetmacro{\SILmax}{-999999}
  \pgfplotstableforeachcolumnelement{Silhouette}\of{\datatable}\as\val{%
    \pgfmathparse{\val}%
    \pgfmathsetmacro{\SILmin}{min(\SILmin,\pgfmathresult)}%
    \pgfmathsetmacro{\SILmax}{max(\SILmax,\pgfmathresult)}%
  }

  \pgfmathsetmacro{\DBmin}{999999} \pgfmathsetmacro{\DBmax}{-999999}
  \pgfplotstableforeachcolumnelement{DaviesBouldin}\of{\datatable}\as\val{%
    \pgfmathparse{\val}%
    \pgfmathsetmacro{\DBmin}{min(\DBmin,\pgfmathresult)}%
    \pgfmathsetmacro{\DBmax}{max(\DBmax,\pgfmathresult)}%
  }

  \pgfmathsetmacro{\CHmin}{999999} \pgfmathsetmacro{\CHmax}{-999999}
  \pgfplotstableforeachcolumnelement{CalinskiHarabasz}\of{\datatable}\as\val{%
    \pgfmathparse{\val}%
    \pgfmathsetmacro{\CHmin}{min(\CHmin,\pgfmathresult)}%
    \pgfmathsetmacro{\CHmax}{max(\CHmax,\pgfmathresult)}%
  }

  \pgfmathsetmacro{\MCDmin}{999999} \pgfmathsetmacro{\MCDmax}{-999999}
  \pgfplotstableforeachcolumnelement{MeanCentroidDist}\of{\datatable}\as\val{%
    \pgfmathparse{\val}%
    \pgfmathsetmacro{\MCDmin}{min(\MCDmin,\pgfmathresult)}%
    \pgfmathsetmacro{\MCDmax}{max(\MCDmax,\pgfmathresult)}%
  }

  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{Silhouette}}{\SILmin}{\SILmax}}]%
    {Silhouette_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMaxFlip{\thisrow{DaviesBouldin}}{\DBmin}{\DBmax}}]%
    {DaviesBouldin_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMax{\thisrow{CalinskiHarabasz}}{\CHmin}{\CHmax}}]%
    {CalinskiHarabasz_N}{\datatable}
  \pgfplotstablecreatecol[create col/expr={\MinMaxFlip{\thisrow{MeanCentroidDist}}{\MCDmin}{\MCDmax}}]%
    {MeanCentroidDist_N}{\datatable}

  \pgfplotstablecreatecol[
    create col/expr={
      (\thisrow{Silhouette_N}+\thisrow{DaviesBouldin_N}+\thisrow{CalinskiHarabasz_N}+\thisrow{MeanCentroidDist_N})/4
    }
  ]{Mean}{\datatable}

  \pgfplotstablesort[
    sort key=Mean,
    sort cmp=float >%
  ]{\ssisorted}{\datatable}

  \pgfplotstablecreatecol[
    create col/expr={\pgfplotstablerow+1}
  ]{Rank}{\ssisorted}

  \pgfplotstabletypeset[
    columns={Rank,Dataset,NumberofClusters,Silhouette,DaviesBouldin,CalinskiHarabasz,MeanCentroidDist,Mean},
    columns/Rank/.style={column name=Rank, column type=r},
    columns/Dataset/.style={string type, column name=Dataset},
    columns/NumberofClusters/.style={column name=Number of Clusters, column type=c},
    columns/Silhouette/.style={column name=Silhouette$\uparrow$, fixed, precision=4},
    columns/DaviesBouldin/.style={column name=Davies--Bouldin$\downarrow$, fixed, precision=4},
    columns/CalinskiHarabasz/.style={column name=Calinski--Harabasz$\uparrow$, fixed, precision=2},
    columns/MeanCentroidDist/.style={column name=Mean Centroid Dist.$\downarrow$, fixed, precision=4},
    columns/Mean/.style={
      column name=Mean$\uparrow$, fixed, precision=4,
      postproc cell content/.append code={%
        \ifnum\pgfplotstablerow=0\relax
          \pgfkeysalso{/pgfplots/table/@cell content/.add={\boldmath }{}}%
        \fi
      }
    },
    every head row/.style={before row=\toprule, after row=\midrule},
    every last row/.style={after row=\bottomrule},
    font=\small
  ]{\ssisorted}

  \endgroup
}%
